Non-rigid 3D motion estimation at high temporal resolution from prospectively undersampled k-space data using low-rank MR-MOTUS

With the recent introduction of the MR-LINAC, an MR-scanner combined with a radiotherapy LINAC, MR-based motion estimation has become of increasing interest to (retrospectively) characterize tumor and organs-at-risk motion during radiotherapy. To this extent, we introduce low-rank MR-MOTUS, a framework to retrospectively reconstruct time-resolved non-rigid 3D+t motion-fields from a single low-resolution reference image and prospectively undersampled k-space data acquired during motion. Low-rank MR-MOTUS exploits spatio-temporal correlations in internal body motion with a low-rank motion model, and inverts a signal model that relates motion-fields directly to a reference image and k-space data. The low-rank model reduces the degrees-of-freedom, memory consumption and reconstruction times by assuming a factorization of space-time motion-fields in spatial and temporal components. Low-rank MR-MOTUS was employed to estimate motion in 2D/3D abdominothoracic scans and 3D head scans. Data were acquired using golden-ratio radial readouts. Reconstructed 2D and 3D respiratory motion-fields were respectively validated against time-resolved and respiratory-resolved image reconstructions, and the head motion against static image reconstructions from fully-sampled data acquired right before and right after the motion. Results show that 2D+t respiratory motion can be estimated retrospectively at 40.8 motion-fields-per-second, 3D+t respiratory motion at 7.6 motion-fields-per-second and 3D+t head-neck motion at 9.3 motion-fields-per-second. The validations show good consistency with image reconstructions. The proposed framework can estimate time-resolved non-rigid 3D motion-fields, which allows to characterize drifts and intra and inter-cycle patterns in breathing motion during radiotherapy, and could form the basis for real-time MR-guided radiotherapy.

==> SupplementaryInformation.tex <==
\clearpage
\noindent {\huge\bfseries Supplementary Figures}


% \subsection{Overview pictures}

% \begin{figure}[h!]
% \centering
%     \includegraphics[width=0.43\textheight]{figures/validation_startstopbreathing.pdf}
%     \caption{Overview of validation of the reconstructed motion-fields, as described in \cref{section:motionreconstructionmethods}. Data is acquired in two breath-holds in different positions, both immediately followed by free-breathing. The breath-hold data is used for image reconstruction, and the free-breathing data is used for motion reconstruction. This setup result in two overlapping points, i.e. where the free-breathing and breath-hold overlap. For validation, the NRMSE between the image reconstruction and the warped image from the motion reconstruction is computed on both overlapping points.}
%     \label{figure:validation_startstopbreathing}
% \end{figure}

% \subsection{Time-resolved 2D reconstruction respiratory motion}

\setsuppvideo
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{SuppInfoVideoS1_2D_TRMRMOTUS_vs_CS2Dt.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} 2D-t compressed sensing reconstruction (left), MR-MOTUS warped reference images (middle), and pixel-wise absolute differences between the two reconstructions (right), as mentioned in \cref{section:2dtreconstructionsmethods} and \cref{section:2dtreconstructionsresults}. The top row shows reconstructions for volunteer 1, and the bottom row for volunteer 2.}
    \label{video:TR2DtvsCS2Dt}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS2_2D_RESP_TR_RankDecomp_vol1.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from 2D time-resolved data, as mentioned in \cref{section:2dtreconstructionsmethods} and \cref{section:2dtreconstructionsresults}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 1. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.}
    \label{video:TR2DtMIO}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS3_2D_RESP_TR_RankDecomp_vol2.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from 2D time-resolved data, as mentioned in \cref{section:2dtreconstructionsmethods} and \cref{section:2dtreconstructionsresults}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 2. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.}
    \label{video:TR2DtMIO_VOL2}
\end{figure}

% \newpage

% \subsection{3D reconstructions respiratory motion}



\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{SuppInfoVideoS4_3D_RESP_RR_vs_MRMOTUS_vol1.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} Respiratory-resolved image reconstruction (Resp. resolved IR, left), MR-MOTUS warped reference images (middle), and pixel-wise absolute differences between the two reconstructions (right), as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The visualization shows data from volunteer 1.}
    \label{video:RRMRMOTUS_vs_RRIR}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{SuppInfoVideoS5_3D_RESP_RR_vs_MRMOTUS_vol2.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} Respiratory-resolved image reconstruction (Resp. resolved IR, left), MR-MOTUS warped reference images (middle), and pixel-wise absolute differences between the two reconstructions (right), as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The visualization shows data from volunteer 2.}
    \label{video:RRMRMOTUS_vs_RRIR_VOL2}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS6_3D_RESP_RR_RankDecomp_vol1.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from respiratory-sorted data, as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 1. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.} 
    \label{video:RR_RankDecomp}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS7_3D_RESP_RR_RankDecomp_vol2.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from respiratory-sorted data, as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 2. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.} 
    \label{video:RR_RankDecomp_VOL2}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS8_3DTR_RankDecomp_vol1.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from respiratory-sorted data, as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 1. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.} 
    \label{video:TR3Dt_Resp_MRMOTUS}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS9_3DTR_RankDecomp_vol2.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images overlayed with reconstructed dynamic motion-fields from respiratory-sorted data, as mentioned in \cref{section:methodsresp3d} and \cref{section:resultsresp3d}. The image shows a decomposition in the reconstructed components $\bm{\Phi}^i$ (spatial) and $\bm{\Psi}$ (temporal) for volunteer 2. For visualization purposes the components were scaled such that $\lVert \bm{\Phi}^i \rVert=1$.} 
    \label{video:TR3Dt_Resp_MRMOTUS_VOL2}
\end{figure}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/3Da_two_positions_coronal.pdf}
%     \caption{Two motion-free images for validation in two different breath-hold positions, as described in \cref{section:motionreconstructionmethods}, \cref{section:methodsresp3d} and \autoref{figure:validation_startstopbreathing}. {\color{red} TO DO: export without cropping black outer border}}
%     \label{fig7}
% \end{figure}

% \newpage
% \setsuppvideo
% \subsection{3D reconstructions head-neck motion}
\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS10_3D_HN_TR_WARPED_vol1.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images resulting from the 3D head-and-neck motion reconstructions for volunteer 1, as mentioned in \cref{section:methodshead3d} and \cref{section:resultshn3d}.} 
    \label{video:TR3Dt_HN_MRMOTUS}
\end{figure}

\begin{figure}[h!]
    \centering        
    \includegraphics[width=\textwidth]{SuppInfoVideoS11_3D_HN_TR_WARPED_vol2.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} MR-MOTUS warped reference images resulting from the 3D head-and-neck motion reconstructions for volunteer 2, as mentioned in \cref{section:methodshead3d} and \cref{section:resultshn3d}.} 
    \label{video:TR3Dt_HN_MRMOTUS_VOL2}
\end{figure}

% \setsuppfig
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/3D_HN_spectrum_reconstructedmf.pdf}
%     \caption{Analysis of the 3D time-resolved head-neck motion-fields with an $R=6$ low-rank motion model as discussed in \cref{section:methodshead3d} and \cref{section:resultshn3d}. (A): Correlation matrix between spatial components $\bm{\Phi}^i$, computed as $|\langle\Phi_i, \Phi_j \rangle|$ with $\lvert\bm{\Phi}^i\rVert =1$. (B): Eigenvalue spectrum. }
%     \label{fig:3D_spectrum_reconstructedmf}
% \end{figure}




% \setsuppfig
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figures/2D_spectrum_reconstructedmf}
%     \caption{Eigenvalue spectrum of the 2D time-resolved motion-fields with an $R=3$ low-rank motion model, as discussed in \cref{section:2dtreconstructionsmethods} and \cref{section:2dtreconstructionsresults}.}
%     \label{fig:2D_spectrum_reconstructedmf}
% \end{figure}
\setsuppvideo
\begin{figure}[h!]
    \centering
    \includegraphics[width=1\textwidth]{SuppInfoVideoS12_3D_RRMRMOTUS_vs_RRIR_4x.pdf}
    \caption{{\it This is an animated figure and should be viewed at \url{https://surfdrive.surf.nl/files/index.php/s/XcXY3cHETnmXtY0}.} Respiratory-resolved image reconstruction (Resp. resolved IR, left), MR-MOTUS warped reference images (middle), and pixel-wise absolute differences between the two reconstructions (right), as mentioned in \cref{section:supp_parametersearch} and \cref{section:methodsresp3d}. The four blocks show reconstructions with different reconstruction parameter settings. `InhaleBinned' denotes whether the reference image is binned in inhale (1) or exhale (0). `Ref. resolution' denotes the resolution of the reference image in millimeters. All motion-fields were reconstructed without regularization and with 9 cubic spline functions in every direction.}
    \label{video:RRMRMOTUS_vs_RRIR_4x}
\end{figure}

\setsuppfig
\begin{figure}[h!]
    \centering
    \includegraphics[width=1.1\textwidth]{SuppInfoFigureS13_2D_snr_comparison.pdf}
    \caption{(A) Roemer reconstruction \citep{Roemer1990}. (B) The coil compression with $\lambda_{CC}=5\cdot 10^5$, as discussed in \cref{section:coilcompression}. (C) SNR loss factor between (A) and  (B). (D) The histogram of the SNR loss factor in (C). The SNR loss factor is between 1.5 and 2.5 in most of the body and increases towards the boundary of the body.}
    \label{fig:2D_snr_comparison}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{SuppInfoFigureS14_3D_reconanalysis.pdf}
    \caption{Results of the parameter search as mentioned in \cref{section:supp_parametersearch} and \cref{section:methodsresp3d}. (A) The effect of the reference image resolution and reference image respiratory binning-phase on the reconstruction quality. (B) The effect of the reference image resolution on the reconstruction time. In the figure, `InhaleBinned' refers to the binning phase for the reference image (InhaleBinned=1 for inhale, InhaleBinned=0 for exhale), `Resolution' denotes the spatial resolution of the reference image, and `SplineOrder' denotes the number of spline basis functions defined per spatial dimension. }
    \label{fig:RR3DtvsRRIR:errorvsresolution}
\end{figure}

